Simplifying Node Classification on Heterophilous Graphs with Compatible Label Propagation

Graph Neural Networks (GNNs) have been predominant for graph learning tasks; however, recent studies showed that a well-known graph algorithm, Label Propagation (LP), combined with a shallow neural network can achieve comparable performance to GNNs in semi-supervised node classification on graphs with high homophily. In this paper, we show that this approach falls short on graphs with low homophily, where nodes often connect to the nodes of the opposite classes. To overcome this, we carefully design a combination of a base predictor with LP algorithm that enjoys a closed-form solution as well as convergence guarantees. Our algorithm first learns the class compatibility matrix and then aggregates label predictions using LP algorithm weighted by class compatibilities. On a wide variety of benchmarks, we show that our approach achieves the leading performance on graphs with various levels of homophily. Meanwhile, it has orders of magnitude fewer parameters and requires less execution time. Empirical evaluations demonstrate that simple adaptations of LP can be competitive in semi-supervised node classification in both homophily and heterophily regimes.

==> pages/discussion.tex <==
\textbf{Comments from Reviewer 2}

Thank you for your detailed suggestions and reviews.

\textbf{1.} ``If my understanding is correct, $\mathbf{I}$ is a matrix (=order-2 tensor) and $\mathbf{I} \odot \mathbf{A}^{\mathbf{F}}$ is an order-3 tensor. Therefore, $\mathbf{I} - \alpha \mathbf{I} \odot \mathbf{A}^{\mathbf{F}}$ is an invalid operation. In addition, It is not obvious how to define the inverse $\cdot^{-1}$ for an order-3 tensor.
I also have several questions about the proof in the appendix. First, given the equation $[\hat{\mathbf{B}}]_{:, k} = (1-\alpha) [\hat{\mathbf{D}}]_{:, k} + \alpha \mathbf{A}^{\mathbf{F}}[\hat{\mathbf{B}}]_{:, k}$, the vectorization operator is applied to it. However, it does not take any effect because both sides are already vectors. In addition, the transformation from eq. (20) to eq. (21) is difficult to interpret because the inverse operator for a rank-3 tensor is not obvious, as I mentioned above.". 

\textcolor{red}{
{\it Our response:}
We are sorry for this confusing part and thank the reviewer for the concrete question.
We have revised Section 5.4 to clarify Proposition 1 and 2, and updated Appendix B to fix the corresponding proofs.
Specifically, CLP iterative update node class label prediction of each class in turn (as shown in Equation (8)), therefore we present Proposition 1 and Proposition 2 for class $k$ and discuss their validity, respectively. 
Similarly, we can easily generalise these propositions to other class labels. 
}

\textbf{2.} ``Regarding Proposition 2, we can only apply the spectral radius operator $\rho(\cdot)$ to a matrix, while $\mathbf{A}^{\mathbf{F}}$ is an order-3 tensor. Therefore it is difficult to interpret $\rho(\mathbf{A}^{\mathbf{F}})$.''

\textcolor{red}{
{\it Our response:}
Thank you for the insightful comments. Following the revision of Proposition 1 (Section 5.4), we have updated Proposition 2 and its proof (Appendix B)
}

\textbf{3.} ``Additional comment: In Eq. (5), Definition of $\mathbf{Y}$ is missing. I guess this is the concatenation of one-hot encoded target labels.''

\textcolor{red}{
{\it Our response:}
We thank the reviewer for this observation. 
The definition of $\mathbf{Y}$ was mistakenly deleted in the previous revision.
We have revised Eq. (5) with the definition of $\mathbf{Y}$. 
}

